Generalized Framework for Group Testing: Queries, Feedbacks and Adversaries

In the Group Testing problem, the objective is to learn a subset K of some much larger domain N, using the shortest-possible sequence of queries Q. A feedback to a query provides some information about the intersection between the query and subset K. Several specific feedbacks have been studied in the literature, often proving different formulas for the estimate of the query complexity of the problem, defined as the shortest length of queries' sequence solving Group Testing problem with specific feedback. In this paper we study what are the properties of the feedback that influence the query complexity of Group Testing and what is their measurable impact. We propose a generic framework that covers a vast majority of relevant settings considered in the literature, which depends on two fundamental parameters of the feedback: input capacity $\alpha$ and output expressiveness $\beta$. They upper bound the logarithm of the size of the feedback function domain and image, respectively. To justify the value of the framework, we prove upper bounds on query complexity of non adaptive, deterministic Group Testing under some "efficient" feedbacks, for minimum, maximum and general expressiveness, and complement them with a lower bound on all feedbacks with given parameters $\alpha,\beta$. Our upper bounds also hold if the feedback function could get an input twisted by a malicious adversary, in case the intersection of a query and the hidden set is bigger than the feedback capacity $\alpha$. We also show that slight change in the feedback function may result in substantial worsening of the query complexity. Additionally, we analyze explicitly constructed randomized counterparts of the deterministic results. Our results provide some insights to what are the most useful bits of information an output-restricted feedback could provide, and open a number of challenging research directions.

==> abstract_short.tex <==
In the Group Testing problem, the objective is to learn a subset $K$ of some large domain $N$, using the shortest-possible sequence of queries. A feedback to a query provides some information about the intersection between the query and set $K$. This paper studies what are the properties of the feedback that influence the query complexity (the length of the query sequence) of Group Testing and what is their measurable impact. We propose a generic framework that covers a vast majority of relevant settings considered in the literature, which depends on two fundamental feedback parameters: input capacity $\alpha$ and output expressiveness $\beta$. They upper bound the logarithm of the size of the feedback function domain and image, respectively. It also contains an adversarial component if the intersection of the query and the set exceeds feedback capacity. To justify the value of the framework, we prove upper bounds on query complexity of non-adaptive, deterministic Group Testing under efficient feedbacks, for minimum, maximum and general expressiveness, and complement them with a lower bound on all feedbacks with given $\alpha$, $\beta$. Our results provide some insights to what are the most useful bits of information an output-restricted feedback could provide.

==> full-feedback-lower-old.tex <==
% !TEX root = general_feedback.tex
\subsection{Full feedback}

We define the following $(\alpha,\alpha\log n)$-feedback function.
%\Marek{Do ujednolicenia} 
\[
F(S) = S.
\]
We will call such feedback function \fullfeed{\alpha}. Here the feedback function returns the set $S$ (understood as the set of identifiers of the elements). Such a set can be encoded using $\alpha\log_2 n$ bits.


\begin{lemma}
\label{lem:fullupper}
If $k < \sqrt{n}$ and $\alpha \geq 18 \log k$, then there exists a family $\mathcal{A}$ of $t=O((k^2 / \alpha^2) \cdot \log (n/k))$ subsets of $N$\Marek{Jest tez niejednoznacznosc z $N$ porownujac z innymi rozdzialami} with the property that for any set $S\subset N$ such that $|S| \leq k$ and any element $s\in S$, there exists  $A \in \mathcal{A}$ with the property that $s \in A$ and $|S \cap A| \leq \alpha$.
\end{lemma}
\begin{proof}


In other words we need to show that there  exists a family of $t$ subsets of $\mathcal{A}$ such that for any  $|S| \leq k$

 Such that if at most $S$ 
We need to show that 
Let  $h =\lceil 32 \log(3n/k) \rceil$. We construct a $6h \cdot k^2 / \alpha^2\times n$ binary matrix, where each entry is $1$ with probability $\frac{\alpha}{6 \cdot k}$ and $0$ otherwise. We will show that there exists a matrix satisfying the following two claims:
\subparagraph{Claim 1} With probability at least $2/3$ each column has at least $\frac{hk}{2\alpha} $ ones.\\
For a fixed column $v$, the number of ones $N_v$ in the column is a sum of Bernoulli random variables. We have $\E{N_v} = \frac{hk}{\alpha}$ hence we can bound the probability that this event fails for a fixed $v$ as follows:
\[
\Pr{N_v < h\frac{k}{2\alpha}} \leq e^{-\frac{hk}{16\alpha}} <\frac{1}{3n},
\]
where the last inequality follows from the fact that, $\frac{hk}{16\alpha} \geq 32 \log(3n/k) / 16  \geq \log(3n) $ (because $k < \sqrt{n}$).



Taking the union bound over all $n$ columns, completes the proof of the claim.
\subparagraph{Claim 2} With probability at least $2/3$ for every subset of $\frac{hk}{2\alpha}$ rows and any subset of $k$ columns, the resulting $\frac{hk}{2\alpha} \cdot \log(n/k) \times k$ matrix has at least one row with at most $\alpha$ ones.

For any fixed subset of $k$ columns and $\frac{hk}{\alpha}$ rows, the number of ones $X_r$ in a row $r$ of the resulting matrix is a sum of $k$ binomial random variables. We have $\E{X_r} = \frac{\alpha}{6}$, we have by Chernoff bound
\[
\Pr{X_r > \alpha} <\Pr{X > 6 \E{X}} < e^{-\alpha}.
\]
The probability that this happens in each of $\frac{hk}{2\alpha}$ rows is at most:
\[
e^{-\alpha \cdot \frac{hk}{2\alpha}} =e^{-\frac{hk}{2}}.
\]
The logarithm of the number of possible combinations of rows and columns in this claim is:
\[
\log \left({n \choose k} \cdot {\frac{6h k^2}{\alpha^2}\choose \frac{hk}{\alpha}}\right) \leq k \log\left(\frac{en}{k}\right) + \frac{hk }{\alpha} \log\left(\frac{6 e k}{\alpha}\right),
\]
and since $\alpha > 18 \log k$, we obtain:
\begin{align*}
\log \left(e^{-\frac{hk}{2}} \cdot {n \choose k} \cdot {6h \cdot \frac{k^2}{\alpha^2}\choose h \cdot \frac{k}{\alpha}}\right) &\leq -\frac{hk}{2}  + k \log\left(\frac{en}{k}\right) + \frac{hk }{\alpha} \log\left(\frac{6 e k}{\alpha}\right)\\
& \leq - \frac{hk}{2}   + k \log\left(\frac{en}{k}\right) + \frac{hk \log k}{18 \log k} \leq -\frac{4hk}{9} + k \log\left(\frac{en}{k}\right) \\
& \leq - 14 k \log\frac{3n}{k} + k\log\frac{en}{k} \leq -13 k\log\frac{3n}{k} < \log\frac{1}{3}.
\end{align*}
Hence:
\[
e^{-k \cdot 32 \log(3n/k)} \cdot {n \choose k} \cdot {\frac{6h k^2}{\alpha^2}\choose \frac{hk}{\alpha}} <\frac{1}{3}.
\]
Thus, by using Union bound this completes the proof of the claim and we observe by using the probabilistic method, that there exists a matrix $M$ satisfying both claims.

To construct a family $A_1, A_2,\dots, A_t$, with $t \in O((k^2 / \alpha^2) \cdot \log (n/k))$ out of the matrix we simply include $i$-th element in set $j$ if entry in $j$-th row and $i$-th column of matrix $M$ is $1$. Claim $1$ implies that each element of $N$ belongs to at least $\frac{hk}{2\alpha}$ sets and claim $2$ implies that regardless of the choice of $K$, every subfamily of $\frac{hk}{2\alpha}$ sets contains a set with at most $\alpha$ elements from $K$. 
\end{proof}

\begin{theorem}
\label{thm:fullupper}
Under the $\fullfeed{\alpha}$ feedback model, if $\sqrt{n} > k > \alpha > 18 \log k$, there exists a  family solving the $k$-group testing problem with $t \in O((k^2 / \alpha^2) \cdot \log (n/k))$.
\end{theorem}
\begin{proof}
The theorem is a direct consequence of Lemma~\ref{lem:fullupper}. We simply observe that under the $\fullfeed{\alpha}$ feedback model, family $\mathcal{A}$ solves the $k$-group testing problem, because the feedback returns at least once the identifier of each element of $S$.
 \end{proof}


==> funding.tex <==
\vspace*{5mm}\\ \textbf{Acknowledgements}
Partially supported by Polish National Science Center (NCN) grants 2019/33/B/ST6/02988 and 2017/25/B/ST6/02553,
%M. Klonowski -- Partially funded by the National Science Centre, Poland - Grant Number ... .... 
%
%D. R. Kowalski -- Partially supported 
and by NSF Secure and Trustworthy Cyberspace Award 2131538.
%
% D. Pajak -- Partially funded by the National Science Centre, Poland - Grant Number 2019/33/B/ST6/02988

==> lower-bound.tex <==
\section{Lower bound}

Consider first a binary feedback, $\beta=1$.

Consider queries $Q_1,\ldots,Q_m$, for some $m=c\cdot \frac{k^2}{\alpha^{3/2}}$, for some constant $c>0$, that solve $(n,k)$-Group-Testing with $\alpha$-oracle and $\beta$-feedback.
We may assume that all queries have more than $1$ element; otherwise, we could exclude the singletons and deal with the remaining queries.
Consider a randomly selected pair $\{v,w\}$ of different elements from $[n]$. 
For any integer $1\le m$, let $X_i(v,w)$ be equal to the size of $Q_i$ if $|Q_i\cap \{v,w\}|=1$ and $0$ otherwise,
and let $Y(v,w)=\{i: X_i(v,w)>0\}$.

\begin{lemma}
\label{l:expectedX}
$E[\sum_{i=1}^m X_i(v,w)] \le ???$ and $E[Y(v,w)] ???$.
\end{lemma}

\begin{proof}
$E[\sum_{i=1}^m X_i(v,w)] = \sum_{i=1}^m |Q_i|\cdot \frac{2|Q_i|(n-|Q_i|)}{n(n-1)}$
\end{proof}

It follows from Lemma~\ref{l:expectedX} and the Markov inequality, that there is a pair $\{v,w\}$ such that
$\sum_{i=1}^m X_i(v,w)] \le ???$ and $Y(v,w) ???$.


